FedZeN: Towards superlinear zeroth-order federated learning via incremental Hessian estimation

Federated learning is a distributed learning framework that allows a set of clients to collaboratively train a model under the orchestration of a central server, without sharing raw data samples. Although in many practical scenarios the derivatives of the objective function are not available, only few works have considered the federated zeroth-order setting, in which functions can only be accessed through a budgeted number of point evaluations. In this work we focus on convex optimization and design the first federated zeroth-order algorithm to estimate the curvature of the global objective, with the purpose of achieving superlinear convergence. We take an incremental Hessian estimator whose error norm converges linearly, and we adapt it to the federated zeroth-order setting, sampling the random search directions from the Stiefel manifold for improved performance. In particular, both the gradient and Hessian estimators are built at the central server in a communication-efficient and privacy-preserving way by leveraging synchronized pseudo-random number generators. We provide a theoretical analysis of our algorithm, named FedZeN, proving local quadratic convergence with high probability and global linear convergence up to zeroth-order precision. Numerical simulations confirm the superlinear convergence rate and show that our algorithm outperforms the federated zeroth-order methods available in the literature.

==> sections/backup.tex <==
\textbf{Contributions}: Motivated by the absence of federated zeroth-order algorithms which leverage the curvature information, in this paper we design a novel algorithm, named FedZeN (Zeroth-order Newton). The distinguishing feature of our algorithm is a randomized incremental estimator of the full Hessian matrix, which is the distributed zeroth-order counterpart of the estimator proposed in \cite{Leventhal_Lewis_2011}. 
The gradient and Hessian estimators are built at the master in a communication-efficient manner, exploiting synchronized pseudo-random number generators to generate a common set of $r$ search direction at all the nodes. If the internal seed of the generators is kept private, this procedure also hides the estimated derivatives from potential external eavesdroppers. At each iteration clients only need to evaluate their local function at $2r+1$ query points and transmit to the central server $2r$ scalar values. Remarkably, the design parameter $r$ is independent from the dimension of the problem, making the algorithm suitable for client devices with limited resources. Moreover, the algorithm can be applied to pools of clients with heterogeneous data distributions and is unaffected by client drift.
The efficient estimation of the global Hessian enables tackling federated optimization problems using second-order methods even when the exact derivatives are not available. Indeed, in FedZeN the master updates the model parameters using a Newton-type method, which is known to be significantly faster than first-order methods. We focus on convex optimization problems, handling the approximation error due to the zeroth-order estimation using either appropriate regularization or an eigenvalue clipping safeguarding.

%%%%%%%%%%%

\begin{figure}[]
  \centering
 
    \begin{subfigure}[b]{\columnwidth}
        \centering
        \parbox{0.8\columnwidth}{          \includegraphics[width=0.8\columnwidth]{fig/FedZeN_vs_nonZO_legend2.pdf}
        }
    \end{subfigure}
     
    \vspace{0.2cm}
    \hfill
    \begin{subfigure}[b]{\columnwidth}
         \centering
         \parbox{0.9\columnwidth}{
              \includegraphics[width=0.95\columnwidth]{fig/Covtype2_FedZeN_vs_nonZO_trainingLoss_iterations.pdf}
         }
     \end{subfigure}

    \caption{Comparison with federated algorithms which use the exact derivatives. We show FedAvg with learning rate $\eta=0.1$, $E=5$ local epochs and batchsize $B=100$. The parameters of FedNL are the ones used in the original paper, namely rank-1 compression operator and stepsize $\alpha=1$. The parameters of FLECS are tuned by trial and error to obtain the best possible performance. GIANT uses backtracking line search.}
    \label{fig:vs_nonZO}  
    
\end{figure}

%%%%%%

\begin{algorithm}
\caption{FedJacobi}\label{alg:FedJacobi}
\begin{algorithmic}
\Initialize{
     Central server (CS): Choose $x_1 \in \mathbb{R}^d$. \\
     Clients: Choose $\mu \geq 0$.
     }
\State % for spacing
\State CS: Broadcast a random seed for the PRNG.
\For{each iteration $k = 1, 2, \dots$}
    \State All nodes: Generate $[u_1 \dots u_r]$ using \eqref{eq:Stiefel}.
    \State CS: Broadcast $x_k$.
    \For{each client $i \in [n]$}
        \State Compute $c_{ij}, b_{ij} \, j \in [d]$ using (\ref{eq:c_ij},\ \ref{eq:b_ij}).
    \EndFor    
    \State CS: $c_{j} = \frac{1}{n} \sum_{i=1}^n c_{ij}, \, b_{j} = \frac{1}{n} \sum_{i=1}^n b_{ij}, \, j \in [d].$
    \State CS: Compute $g_k$ using \eqref{eq:gradient_estimator_federated}, $H_k = \sum_{j=1}^d b_j \left( u_j u_j^T \right)$.
    \State CS: $x_{k+1} = x_k - \alpha H_k^{-1} g_k$.
\EndFor
\end{algorithmic}
\end{algorithm}


Federated learning is a distributed learning framework that allows a set of clients to collaboratively train a model under the orchestration of a central server, without sharing raw data samples.
Although in many practical scenarios the derivatives of the objective function are not available, only few works have considered the federated zeroth-order setting, in which functions can only be accessed through point evaluations. In this work we focus on convex optimization and design a novel federated zeroth-order algorithm, which is the first to estimate and exploit the curvature of the global objective.
Our randomized derivative estimators are built at the central server in a communication-efficient and privacy-preserving way by leveraging synchronized pseudo-random number generators. In particular, the Hessian estimator is incrementally updated and the search directions are sampled from the Stiefel manifold.
The numerical simulations show that our algorithm, named FedZeN, outperforms the federated zeroth-order methods available in the literature.

Differently from previous works about federated zeroth-order optimization, which only exploit gradient estimates, here we focus on convex optimization and estimate also the Hessian matrix with the purpose of achieving superlinear convergence.
In particular we take an incremental randomized estimator that converges linearly to the exact Hessian, and we adapt it to the federated zeroth-order setting.
